Primal Dual Affine Scaling on GPUs

Here we present an implementation of Primal-Dual Affine scaling method to solve linear optimization problem on GPU based systems. Strategies to convert the system generated by complementary slackness theorem into a symmetric system are given. A new CUDA friendly technique to solve the resulting symmetric positive definite subsystem is also developed. Various strategies to reduce the memory transfer and storage requirements were also explored.

==> EXP.tex <==
$$\begin{bmatrix}
  0  &0 &a11 &a12 &a13  &0  &0  &0\\
  0  &0 &a21 &a22 &a23  &0  &0  &0\\
a11 &a21  &0  &0  &0  &1  &0  &0\\
a12 &a22  &0  &0  &0  &0  &1  &0\\
a13 &a33  &0  &0  &0  &0  &0  &1\\
  0  &0  &1  &0  &0  &d1  &0  &0\\
  0  &0  &0  &1  &0  &0  &d2  &0\\
  0  &0  &0  &0  &1  &0  &0  &d3
\end{bmatrix}
\begin{bmatrix}
-&-&-&-&-&-&-&-\\
-&-&-&-&-&-&-&-\\
\frac{1}{3a11}&\frac{1}{3a21}&-&-&-&-&-&-\\
\frac{1}{3a12}&\frac{1}{3a22}&-&-&-&-&-&-\\
\frac{1}{3a13}&\frac{1}{3a23}&-&-&-&-&-&-\\
-&-&-&-&-&-&-&-\\
-&-&-&-&-&-&-&-\\
-&-&-&-&-&-&-&-
\end{bmatrix}
=
\begin{bmatrix}
1&0&0&0&0&0&0&0\\
0&1&0&0&0&0&0&0\\
0&0&1&0&0&0&0&0\\
0&0&0&1&0&0&0&0\\
0&0&0&0&1&0&0&0\\
0&0&0&0&0&1&0&0\\
0&0&0&0&0&0&1&0\\
0&0&0&0&0&0&0&1
\end{bmatrix}
$$
$$
Z=\begin{bmatrix}
O&A&O\\
A^T&O&I\\
O&I&D
\end{bmatrix}$$
$$Z^{-1}=\begin{bmatrix}
(ADA^T)^{-1}&(ADA^T)^{-1}AD&-(ADA^T)^{-1}A\\
DA^T(ADA^T)^{-1}&DA^T(ADA^T)^{-1}AD-D&I-DA^T(ADA^T)^{-1}A\\
 -A^T(ADA^T)^{-1} &\left[I-DA^T(ADA^T)^{-1}A\right]^T&A^T(ADA^T)^{-1}A
\end{bmatrix}$$
$$Z*Z^{-1}=\begin{bmatrix}

\end{bmatrix}$$

==> badSimplex.tex <==
Time taken by a linear programming algorithm is measured in terms of the no of components of variable $\mathbf{x} \in \mathbb{R}^n$. Simplex method have been shown to have exponential worst case complexity by Klee and Minty  \cite{KleeMinty:1970}. A simple example for which the worst case behavior occurs is presented here 
\begin{align*}
maximize~&c^Tx \\
&Ax\leq b\\
&x\geq0
\end{align*}
$$c=
\begin{bmatrix}
10^{n-1}\\
10^{n-2}\\
\vdots\\
10^{0}
\end{bmatrix}
b=
\begin{bmatrix}
10^0\\
10^2\\
\vdots\\
10^{2(n-1)}
\end{bmatrix}
$$$$
A=
\begin{bmatrix}
1&0&\cdots&0&0\\
2\times 10^1&1&\cdots&0&0\\
2\times 10^2&2\times 10^1&\cdots&0&0\\
\vdots&\vdots&&\vdots&\vdots\\
2\times 10^{n-1}&2\times 10^{n-2}&\cdots&2\times 10^1&1\\
\end{bmatrix}
$$
The example is from Chong \cite{Chong:2008fk}. Simplex algorithm applied to the above problem requires 2$^n$-1 steps to find the solution. This Problem is an example of worst case of simplex algorithm and clearly we can see that in worst case, simplex algorithm has O($2^n$) time complexity or so said to have exponential complexity.But interior point methods have polynomial convergence. Study of interior point methods began with work of Karmakar \cite{Karmakar:1984} and the area now has well established theoretical background. Some of the most widely used interior point methods can be found in Saigal \cite{Saigal:1995,Saigal:1994,Saigal:1993} as well as Chong \cite{Chong:2008fk}and Nazareth \cite{Nazareth:2004}.
